Floquetifying stabiliser codes with distance-preserving rewrites

Stabiliser codes with large weight measurements can be challenging to implement fault-tolerantly. To overcome this, we propose a Floquetification procedure which, given a stabiliser code, synthesises a novel Floquet code that only uses single- and two-qubit operations. Moreover, this procedure preserves the distance and number of logicals of the original code. The new Floquet code requires additional physical qubits. This overhead is linear in the weight of the largest measurement of the original code. Our method is based on the ZX calculus, a graphical language for representing and rewriting quantum circuits. However, a problem arises with the use of ZX in the context of rewriting error-correcting codes: ZX rewrites generally do not preserve code distance. Tackling this issue, we define the notion of distance-preserving rewrite that enables the transformation of error-correcting codes without changing their distance. These distance-preserving rewrites are used to decompose arbitrary weight stabiliser measurements into quantum circuits with single- and two-qubit operations. As we only use distance-preserving rewrites, we are guaranteed that a single error in the resulting circuit creates at most a single error on the data qubits. These decompositions enable us to generalise the Floquetification procedure of [arXiv:2307.11136] to arbitrary stabiliser codes, provably preserving the distance and number of logicals of the original code.

==> sections/extended-abstract.tex <==
\noindent \textbf{Link} \href{https://arxiv.org/abs/2410.17240}{https://arxiv.org/abs/2410.17240} (alternatively, see attached)


\noindent \textbf{TL;DR} Stabiliser codes with large weight measurements can be challenging to implement fault-tolerantly.
To overcome this, we propose a Floquetification procedure which, given a stabiliser code, synthesises a novel Floquet code that only uses single- and two-qubit operations.
Moreover, this procedure preserves the distance and number of logicals of the original code.
The new Floquet code requires additional physical qubits.
This overhead is linear in the weight of the largest measurement of the original code.

For this procedure, we formalise the space of steps allowed in order to preserve the error correction capabilities of the code.
This builds a formal foundation to understand existing procedures, e.g. those proposed by \parencite{bombinUnifyingFlavorsFault2024, townsend-teagueFloquetifyingColourCode2023}.

\noindent \textbf{Background} One major challenge of quantum computing is dealing with noise~\parencite{gottesmanStabilizerCodes1997}.
The goal of quantum error correction is to encode data with sufficient redundancy to detect and correct errors.
A class of error-correcting codes are stabiliser codes~\parencite{gottesmanStabilizerCodes1997}.
Stabiliser codes are defined by a set of commuting Pauli measurements.
They encode logical qubits into a larger physical space where the code space is the subspace stabilised by the Pauli measurements. 
This defines a static stabilising group through which codes are usually studied.

Floquet codes~\parencite{hastingsDynamicallyGenerated2021,vuillotPlanarFloquet2021} are a recently discovered class of error-correcting codes that allow non-commuting measurements, resulting in an evolving stabiliser group. 
We study these codes via their measurement circuit obtained by repeating their syndrome measurements.

\noindent \textbf{Contribution}  
We leverage this circuit-centric view of Floquet codes to synthesise new error-correcting codes from existing ones.
Given an arbitrary stabiliser code, we derive a new Floquet code that uses operations of weight at most two while preserving the distance and number of encoded logical qubits.
This process generalises the Floquetification procedure proposed by \textcite{townsend-teagueFloquetifyingColourCode2023} to arbitrary stabiliser codes while lowering the qubit overhead. 

Our method is based on the ZX calculus~\parencite{coeckeInteractingQuantumObservables2008}, a graphical language for representing and rewriting quantum circuits.
However, a problem arises with the use of ZX in the context of rewriting error-correcting codes: ZX rewrites generally do not preserve code distance.
Tackling this issue, we define the notion of \emph{distance-preserving rewrite} that enables the transformation of error-correcting codes without changing their distance.

We use these distance-preserving rewrites to decompose stabiliser measurements into quantum circuits with single- and two-qubit operations.
As we only use distance-preserving rewrites, we are guaranteed that a single error in the resulting circuit creates at most a single error on the data qubits.
These decompositions enable us to provide a Floquetification procedure for arbitrary stabiliser codes, provably preserving the distance of the original code.

\noindent \textbf{Distance-preserving rewrites} (\autoref{sec:distance-preservation}) 
% ZX errors
In quantum circuits, one can assume different noise models such as phenomenological noise or circuit-level noise. 
On ZX diagrams, we similarly have to define what we mean by an error. 
An atomic error, which we call \textit{edge flip}, consists of a single Pauli error added to an edge of a ZX diagram. 
For example, we might have:
\[
 \tikzfig{prerequisites/error-example-base}\ +\ ((6,7), X)
 \qquad = \qquad
 \tikzfig{prerequisites/edge-flip-example}
\]

\noindent Then, we define an error on a ZX diagram as follows:
\begin{customdef}{2.5}[Error]
 An error ${E}$ in a ZX diagram $D$ is a set of edge flips ${E} = \{(e_1, t_1), \dots, (e_n, t_n)\}$, each in $D$.
 The weight of the error is given by the number of edges affected by ${E}$, i.e.\@ $wt({E}) = |\{e \ |\ (e, t) \in {E}\}|$.
\end{customdef}

% ZX distance
\noindent Paralleling the notion of code distance, we introduce \textit{ZX distance}: 
\begin{customdef}{3.1}[ZX distance]
 Given a ZX diagram $D$, the ZX distance of $D$ is the minimum weight of all non-trivial, undetectable errors.
\end{customdef}

\noindent With this, we can relate ZX distance to the distance of quantum error-correcting codes. 
In particular, we show that the ZX distance gives a lower bound for the code distance of Floquet codes (\autoref{prop:process-distance-proof}) and both distances are the same for stabiliser codes (\autoref{prop:stabiliser-distance-proof}).

We use these two observations to manipulate error correction codes without affecting their distance; 
given a stabiliser code, the ZX distance of the measurement circuit is the same. 
If the rewrites of the measurement circuit preserve the distance of the diagram, we obtain a lower bound for the distance for any Floquet code we later extract. 

For this, we define: 
\begin{customdef}{3.4}[Distance-preserving rewrite]
A rewrite $r: D_1 \to D_2$ is \emph{distance-preserving} if for all diagrams $D$ in which $D_1$ occurs, we have:
\[\tikzfig{extended-abstract/dist-preservation}\]
\end{customdef}

\noindent While this definition of ZX rewrites quantifies over all possible contexts a rewrite could occur in, we also provide a sufficient condition for distance-preservation that can be verified locally (\autoref{prop:dist-preservation}).

We then find a set of distance-preserving rewrites, including:
\[\tikzfig{extended-abstract/dist-example}\]

\noindent \textbf{Decomposing high-weight measurements} (\autoref{sec:rewriting-measurements})
We use the proposed distance-preserving rewrites to decompose arbitrary-weight Pauli measurements:

\begin{customprop}{5.1}[Decomposing Pauli measurements]
 Any Pauli measurement can be rewritten to get an equivalent diagram consisting only of single- and two-qubit operations using only distance-preserving rewrites.
\end{customprop}

\noindent For example, we have:
\begin{customex}{5.2}[Distance-preserving implementation of a weight-four Pauli measurement]
    \[\tikzfig{extended-abstract/weight-four}\]
 Which is equivalent to the following quantum circuit on six qubits:
    \[\tikzfig{extended-abstract/weight-four-circuit}\]
\end{customex}

\noindent As we restrict ourselves to distance-preserving rewrites, any undetectable error creates at most an error of the same weight on the data qubits and/or a flip of the classical measurement outcome. 
The overhead to implement a weight-$n$ Pauli measurement is at most $\lceil \frac{n}{2} \rceil + \log_{2}{n}$ ancilla qubits. 

\noindent \textbf{Floquetification of stabiliser codes} (\autoref{sec:rewriting})
Using the decomposition of Pauli measurements, we define the Floquetification procedure for arbitrary stabiliser codes.
 For instance, for the $\code{4, 2, 2}$~code, the Floquetification procedure looks as follows: 
 \begin{center}
    \resizebox{\columnwidth}{!}{
        \tikzfig{extended-abstract/extended-abstract-floquetification}
 }
 \end{center}
 
 \noindent  This creates a new Floquet code on six qubits with the same distance as the original code while preserving the number of encoded qubits (\autoref{sec:logical-qubits}). 
 Therefore, we have synthesised a $\code{6, 2, 2}$ Floquet code that only uses measurements of weights one and two. 

 This procedure generalises to arbitrary stabiliser codes. In particular, it transforms any $\code{n, k, d}$ stabiliser code with Pauli measurements of weight at most $m$ into a new $\code{n + \lceil \frac{m}{2} \rceil + \ell, k, d}$ Floquet code with only single- and two-qubit operations where $\ell \leq \log_{2}{m}$.

 Utilising this framework, we can understand the Floquetification of \textcite{townsend-teagueFloquetifyingColourCode2023} as a version of this procedure with delayed qubit reuse. 
 The temporal shift of the time axis reduces to OCM, a distance-preserving rewrite.

 \noindent \textbf{Conclusion} In this paper, we introduce the notion of distance-preserving rewrites to manipulate measurement circuits of quantum error correction codes in the ZX calculus. 
 This allows us to synthesise new codes with desirable properties (in our case low weight measurements) from existing ones while preserving distance and number of encoded logicals. 

 We believe that distance-preserving rewrites can be extended to other areas in fault-tolerant computation such as circuit synthesis and verification.
Building this bridge requires formalising faults in the ZX calculus and extending the distance-preserving rewrite system.
This can lead to novel techniques in fault-tolerant state-preparation and syndrome-extraction.
